Connecting Context-specific Adaptation in Humans to Meta-learning

Cognitive control, the ability of a system to adapt to the demands of a task, is an integral part of cognition. A widely accepted fact about cognitive control is that it is context-sensitive: Adults and children alike infer information about a task's demands from contextual cues and use these inferences to learn from ambiguous cues. However, the precise way in which people use contextual cues to guide adaptation to a new task remains poorly understood. This work connects the context-sensitive nature of cognitive control to a method for meta-learning with context-conditioned adaptation. We begin by identifying an essential difference between human learning and current approaches to meta-learning: In contrast to humans, existing meta-learning algorithms do not make use of task-specific contextual cues but instead rely exclusively on online feedback in the form of task-specific labels or rewards. To remedy this, we introduce a framework for using contextual information about a task to guide the initialization of task-specific models before adaptation to online feedback. We show how context-conditioned meta-learning can capture human behavior in a cognitive task and how it can be scaled to improve the speed of learning in various settings, including few-shot classification and low-sample reinforcement learning. Our work demonstrates that guiding meta-learning with task information can capture complex, human-like behavior, thereby deepening our understanding of cognitive control.

==> archive/babyai.tex <==
\subsection{Sparse-Reward Navigation with BabyAI}

Having established the usefulness of our approach on a toy setup, we now test the generality of our approach on the more challenging task integrating visual information to act as a cue for the goal. 
%
The overarching navigational setup we use for our experiments is the BabyAI research platform, which integrates the use of natural language and agent actions. In BabyAI, the agent is limited by the surrounding walls and field of view, and thus, must rely on exploration and external stimuli to accomplish its mission, which includes ``Pick up the Purple Box" and ``Go to Red Ball". Furthermore, the reward is only delegated upon mission completion, with reward assigned as $ 1 - \frac{n_{steps}}{n_{max}} $. Since this setting is that of sparse-rewards, learning the optimal policy is even more difficult. 

To guide meta-learning in this setting, we study how language can be used as side information to reduce the ambiguity surrounding sparse tasks. We firstly reformulate BabyAI as a meta-learning setup, where different tasks are performed on the same environment but with different seeds and goals (e.g. location and color of objects, direction, initial position of the agent). The resulting variability across tasks induces ambiguity about the correct task-specific policy and mission. 
We then use two BabyAI's environments, Unlock and PutNext, and use the instructions provided to the agent as side information to help it successfully learn across varying tasks. 

In our experiments, we release and withhold contextual information from the pre-adapted network and hypernetwork as dynamic and static contexts. For example, if the agent's mission is to ``Open the Red Door", the agent only knows to ``Open Door" across tasks (static context) but does not know the specific color of the door (dynamic context). Hence, to generate dynamic contexts, we map the task's specific mission (a sentence) to a dictionary of learnable embeddings. For static contexts, however, only the general words such as ``Open" and ``Door" receive learnable embeddings, while specific words are replaced with ones.

%In navigation-based tasks, the POMDP assumption oftentimes limits the rate of learning. For example, in VizDoom, the agent can only observe the screen buffer, and, without general context of the maze, performing well in such an environment is difficult.

==> archive/exp_babyai.tex <==
\pgfplotsset{
  avg-return/.style={
    legend style={
      font=\tiny,
      align=left,
      column sep=3pt,
      nodes={right},
      legend pos=south east,
    },
    y label style={align=center,font=\bfseries\footnotesize,yshift=-5pt},
    x label style={font=\bfseries\footnotesize},
    tick label style={font=\footnotesize},
    enlarge x limits=false,
    grid=major,
    scale only axis,
    restrict y to domain=0:1,
  },
}

\begin{figure*}[t]
\begin{tikzpicture}%
    \begin{axis}[%
      avg-return,
      width=.3\textwidth,
      height=.25\textwidth,
      xlabel={number of timesteps},
      xmin=0, xmax=25000000,
      ymin=0, ymax=1,
      ylabel={average return over tasks},
    ]

    \errorband{data/rl/unlock/unlock_promp.csv}{timesteps}{mean}{std}{black}{0.2}
    \errorband{data/rl/unlock/unlock_static.csv}{timesteps}{mean}{std}{blue}{0.2}
    \errorband{data/rl/unlock/unlock_dynamic.csv}{timesteps}{mean}{std}{red}{0.2}

    \end{axis}
\end{tikzpicture}%
%
\hspace{-9pt}
%
\begin{tikzpicture}%
  \begin{axis}[%
    avg-return,
    width=.3\textwidth,
    height=.25\textwidth,
    xlabel={number of timesteps},
    xmin=0, xmax=25000000,
    ymin=0, ymax=1,
    legend pos=outer north east,
  ]

    \errorband{data/rl/put-next/pro-mp-seed=2.csv}{n_timesteps}{Step_0-AverageReturn}{Step_0-StdReturn}{black}{0.2}
      \addlegendentry{no context, no adaptation \\ (\emph{global parameter baseline})}

    \errorband{data/rl/put-next/pro-mp-seed=2.csv}{n_timesteps}{Step_1-AverageReturn}{Step_1-StdReturn}{black!15!green}{0.2}
      \addlegendentry{no context, w/ adaptation \\ (\emph{\acrshort{promp}~\cite{rothfuss2019promp} baseline})}

    \errorband{data/rl/put-next/dynamic-context-seed=2.csv}{n_timesteps}{Step_0-AverageReturn}{Step_0-StdReturn}{orange}{0.2}
      \addlegendentry{context, no adaptation \\ (\emph{context baseline})}

    \errorband{data/rl/put-next/static-context-seed=2.csv}{n_timesteps}{Step_1-AverageReturn}{Step_1-StdReturn}{blue}{0.2}
      \addlegendentry{static context w/ adaptation \\ (\emph{extra-parameter baseline})}

    \errorband{data/rl/put-next/dynamic-context-seed=2.csv}{n_timesteps}{Step_1-AverageReturn}{Step_1-StdReturn}{red}{0.2}
      \addlegendentry{contextual adaptation \\ (\textbf{ours})}

  \end{axis}
\end{tikzpicture}%
\caption{
    \todo{finish caption}
    (Left) 
    \texttt{Unlock}.
    (Right) 
    \texttt{PutNext}.
}
\label{fig:mujoco}
\end{figure*}


==> archive/intro.tex <==
%file containing the intro used for the ICML submission

Everyday life presents us with a wide range of problems with varying mental demands. A remarkable feature of the human cognitive system is its ability to adapt its decision-making behavior even in the face of such variability~\citep{botvinick2001conflict}. An extensive literature in psychology and neuroscience suggests that task-specific \emph{contextual cues} are crucial in helping people structure their learning in novel situations~\citep{monsell1996control, dosenbach2006core, collins2012reasoning, collins2013cognitive}. In particular, contextual information such as visual or linguistic cues enables people to recognize the underlying structure of the problem at hand, which in turn enables them to decide on a strategy for interaction within the novel context (see Figure \ref{fig:explain}(b) for an example). This context-sensitivity is critical to \emph{cognitive control}--the cognitive processes behind human adaptability~\citep{botvinick2001conflict, botvinick2014computational} and enables efficient learning from a limited amount of data~\citep{collins2012reasoning, collins2013cognitive, werchan20158}.

Similar aims of adaptability and learning efficiency have motivated the development of \emph{meta-learning} algorithms that ``learn how to learn.'' These algorithms emulate the ability of humans to learn from very few examples by pooling information across contexts~\citep{schmidhuber1987evolutionary, thrun1998learning, hochreiter2001learning}, formulated in recent works as the learning of global parameters that are shared between independent, task-specific models~\citep[\eg][]{vinyals2016matching,ravi2017optimization,finn2017model}.

However, one drawback of meta-learning algorithms is that they do not use contextual cues  -- while people shape their learning in a new domain on the basis of the context in which they are learning, meta-learning algorithms treat each task as a random draw from the underlying task distribution (also refer to Figure \ref{fig:explain}(a)). In other words, meta-learning algorithms, unlike humans, learn in the absence of abstract task information and do not provide guidance on how to make the best use of the few samples from the new task.

In this work, we explore settings in which this deficiency plays out strongly, namely when the task distribution is varied or the best predictor is ambiguous given only limited samples from the new task. We integrate contextual cues about task structure--termed \emph{task information}--into meta-learning by augmenting a gradient-based meta-learning algorithm with a \emph{context network} that learns the relationship between task information and initializations of task-specific models. The context-conditional initialization in turn allows the meta-learned prior over task structures to be informed by the task information, similar to how humans guide  learning by context. We show how this approach of \emph{context-conditioned adaptation}--as opposed to either solely conditioning on contextual information, or adapting the task-specific models during interaction--can be applied to both supervised and reinforcement learning tasks. 


\paragraph{Meta-learning.}
Meta-learning aims to learn a model suitable for a distribution of tasks and that enables few-shot adaptation to new tasks~\citep{schmidhuber1987evolutionary,bengio1992optimization,thrun1998lifelong}. While various approaches to meta-learning exist, such as metric-based~\citep[\eg][]{vinyals2016matching,snell2017prototypical} and model-based meta-learning~\citep[\eg][]{santoro2016meta,duan2016rl,wang2016learning}, we focus on gradient-based meta-learning, which comprises an outer loop optimization procedure that learns good initializations for task-specific models that are adapted in an inner loop of optimization~\citep{bengio1992optimization,finn2017model}. Recent work has built upon \gls{gbml} by using probabilistic inference~\citep{grant2018recasting,finn2018probabilistic} or low-dimensional embeddings of task-specific parameters~\citep{rusu2018meta}, or by factorizing parameters into task-specific and task-independent sets~\citep{zintgraf2019caml}. While the general approach of \gls{gbml} applies to a wide variety of problems, the problem setting differs in that it does not provide contextual cues, and thus cannot investigate an analogy of human cognitive control.

Formally, defining $\mathcal{L}_{\mathcal{D}}(f_{\taskparams})$ to be the 
empirical risk of the function $f$ with task-specific parameters $\taskparams$ on the dataset $\mathcal{D}$, $\frac{1}{N}\sum_{(\mathbf{x}, \mathbf{y}) \in \mathcal{D}}[\ell(f_{\taskparams}(\mathbf{x}), \mathbf{y})]$, and setting $\taskparams$ to be the result of a single gradient step initialized at $\metaparams$, the objective that \gls{maml} optimizes is
\begin{equation}\label{eq:maml}
\min_{\metaparams}\  
\mathbb{E}_{\task_j \sample p(\task)}\left[
\mathcal{L}_{\mathcal{D}^\text{q}\taskidx{j}} \left(
f_{\metaparams - \nabla_{\metaparams}{ \big[\mathcal{L}_{\mathcal{D}^\text{s}\taskidx{j}}(f_{\metaparams})\big]
}}
\right)\right]~,
\end{equation}

where the task-specific dataset $\mathcal{D}\taskidx{j}$ is partitioned into disjoint \textbf{s}upport and \textbf{q}uery sets, $\mathcal{D}\taskidx{j} = \mathcal{D}^\text{s}\taskidx{j} \cup \mathcal{D}^\text{q}\taskidx{j}$. While we write the objective for gradient-based adaptation assuming a single step on a supervised learning objective for simplicity, multi-step variants and generalizations to policy search in \gls{rl} are possible~\citep[see][and Section \ref{sec:method} for details]{finn2017model}. As long as the gradient itself is differentiable, $\metaparams$ can be optimized by backpropagation through this global objective function.

In the \gls{maml} algorithm, the task-specific parameters $\taskparams$ are computed via gradient descent on the support-set loss $\mathcal{L}_{\mathcal{D}^\text{s}}$ from initialization $\metaparams$ (\ie in Equation~\ref{eq:maml}, we take $f_{\taskparams}:=f_{\metaparams - \nabla_{\metaparams}{ \big[\mathcal{L}_{\mathcal{D}^\text{s}\taskidx{j}}(f_{\metaparams})\big]}}$ reflecting a single gradient step away from $\metaparams$). The \gls{maml} procedure can be viewed as a choice of implementation of the function $h_{\metaparams} : \mathcal{D}\taskidx{j} \to \taskparams$ that can be straightforwardly augmented with task information in order to improve few-shot learning in ambiguous or low-sample domains, as we will see in Section \ref{sec:method}.

In many cases, the task-specific predictive distribution can be written as $\ell(f_{\taskparams}(\hat{\mathbf{x}}), \hat{\mathbf{y}})$ for loss $\ell$ and mapping $f$ parameterized by task-specific $\taskparams_j$, which are produced as the output of a function $h_{\metaparams}(\mathcal{D}\taskidx{j})$ that conditions on the task-specific dataset $\mathcal{D}\taskidx{j}$~\citep{gordon2018meta}, a perspective that we also adopt.

One particular family of parametric meta-learning approaches known as \gls{gbml} aims to learn a good initial state for task-specific models that are independently adapted with gradient descent~\citep[\eg][]{ravi2017optimization,finn2017model}. The shared initialization makes it easier for each task-specific model to be adapted to a particular solution and therefore acts in the form of a learned prior distribution over task structures~\citep{grant2018recasting}. A popular and straightforward \gls{gbml} approach is the \gls{maml} algorithm~\citep{finn2017model}, in which a common parameter initialization for gradient-based optimization is shared uniformly among all task-specific models; the optimization of the task-specific losses are simply truncated after a fixed number of steps. 


==> archive/safeintro.tex <==
Everyday life presents us with a wide range of problems with varying mental demands. A remarkable feature of the human cognitive system is its ability to adapt its decision-making behavior even in the face of such variability~\citep{botvinick2001conflict}. Similar aims of adaptability and learning efficiency have motivated the development of \emph{meta-learning} algorithms that ``learn how to learn.'' These algorithms emulate the ability of humans to learn from very few examples by pooling information across contexts~\citep{schmidhuber1987evolutionary, thrun1998learning, hochreiter2001learning}, formulated in recent works as the learning of global parameters that are shared between independent, task-specific models~\citep[\eg][]{vinyals2016matching,ravi2017optimization,finn2017model}. 

Yet, despite these successes, current meta-learning approaches still fall short of the kind of efficiency and adaptability exhibited by humans. While there are a number of reasons behind this, this paper considers one prominent feature of human adaptability -- the importance of task-specific \emph{contextual cues} in helping people structure their learning in novel situations~\citep{monsell1996control, dosenbach2006core, collins2012reasoning, collins2013cognitive}. As an example, consider Alice who is learning how to operate a new tool and Bob who is learning how to play a new instrument. Even before Alice and Bob begin to learn their respective tasks, task information in the form of visual cues (such as the image of the tool/instrument) or linguistic cues (such as descriptions about the task) inform them about the structure of the policy space. In essence, contextual information such as visual or linguistic cues enable people to recognize the underlying structure of the problem at hand, which in turn enables them to decide on a strategy for interaction within the novel context (see Figure \ref{fig:explain}(b) for another example).

Current meta-learning approaches, on the other hand, learn in the absence of abstract task information by treating each task as a random draw from the underlying task distribution. As a consequence, they do not utilize guidance on how to make the best use of the few samples from the new task (also refer to Figure \ref{fig:explain}(a)). Expanding on the above Alice and Bob example, Alice and Bob would differ in their respective priors whereas a meta-learning algorithm would apriori treat both tasks equally thereby leading to decreased sample efficiency. 

In this work, we explore settings in which this deficiency plays out strongly, namely when the task distribution is varied or the best predictor is ambiguous given only limited samples from the new task. We integrate contextual cues about task structure--termed \emph{task information}--into meta-learning by augmenting a gradient-based meta-learning algorithm with a \emph{context network} that learns the relationship between task information and initialization of task-specific models. The context-conditional initialization in turn allows the meta-learned prior over task structures to be informed by the task information, similar to how humans guide  learning by context (also refer to Figure \ref{fig:explain}(c)). We show how this approach of \emph{context-conditioned adaptation}--as opposed to either solely conditioning on contextual information, or adapting the task-specific models during interaction--can be applied to improve the speed of learning for both supervised (sinusoid regression and CIFAR dataset) and reinforcement learning (MuJoCo and Meta-World) tasks. 

To summarize, our key contributions are as follows: 

\begin{itemize}
    \item Analogous to human learning, we introduce a framework to use task information to guide the initialization of task-specific models before adaptation to online feedback. 
    
    \item In contrast to prior on context-conditioned meta-learning that primarily produce the task-encoding using the \emph{same} data as the meta-learner \citep{oreshkin2018tadam, pahde2018cross, vuorio2018toward, chen2019adaptive, lee2018gradient, lee2019learning, baik2019learning, lan2019meta, yoon2019tapnet}, we demonstrate the value of utilizing the \emph{extra} available contextual information to improve the performance of meta-learning.
    
    \item We offer extensive experiments by evaluating our model against rigorous baselines and show that our method improves the speed of learning on a variety of supervised and reinforcement learning benchmarks.
\end{itemize}


==> archive/sinusoid.tex <==
\subsection{Supervised learning warm-up: Ground-truth task information in sinusoid regression}
\label{sec:sinusoid}

We begin our evaluation by conducting experiments on a simple supervised learning task in the form of sinusoid regression, inspired by the task originally used to demonstrate the utility of \gls{maml}~\citep{finn2017model}.
 
%This experiment evaluates whether context-conditioned adaptation is helpful when interaction with the task is less adequate to resolve ambiguities about its underlying structure.
Further, this experiment examines whether the particular way of implementing context-conditioning introduced in Section \ref{sec:method} has the potential to outperform other strong baselines.

\paragraph{Experimental setup.}
We define each task of regressing to a sine curve by uniformly sampling the amplitude from $[0.  1, 5.  0]$ and the phase from $[0, \pi]$.
We use the amplitude and phase as the task information for this setting.
While we expect access to this task information to improve performance, our goal is to evaluate whether context-conditioning performs better than simply feeding the context as an extra input to the base network (\ie \gls{maml-concat}).

\paragraph{Hyperparameters.}
For both the base and context networks, we use a neural network with two hidden layers each of dimension 40, similarly to \cite{finn2017model}.
Note that, for this experiment the dimensionality of $\metaparams$ is sufficiently low that we do not need to use the \gls{film} parameterization for the output of the context network.
Instead, we have the context network output $\metaparams$  directly, learning a function from task information to the initial weights of the base network; more details on the implementation of the context network can be found in Appendix \ref{sec:exp_details}.
For gradient-based adaptation during meta-training, for each task we use one gradient update using a support set of size $10$; during meta-evaluation we present the model with $10$ support examples from a newly sampled task and measure mean-squared error over $256$ query set examples.
 
\paragraph{Results.}
As shown in Figure~\ref{fig:regression}, we see that, as expected, task information reduces ambiguity in sinusoid regression as both \gls{maml-context} and \gls{maml-concat} significantly outperform \gls{maml}.
We also note that while \gls{maml-static} performs better than \gls{maml} due to the increase in parameters and therefore expressivity, its performance is worse than \gls{maml-context} and \gls{maml-concat}.
Lastly, we see that the \gls{maml-context} method outperforms the \gls{maml-concat} method, suggesting that even in a toy setup, context-conditioning is  more useful than simply providing the context as an extra input to \gls{maml}.

\paragraph{Ablation.} 
We next investigate the effect of ablating the amount of context that is provided to \Gls{maml-concat} and \gls{maml-context} where we provide only one of the phase or amplitude as task information (refer to Figure \ref{fig:regression_ablation}).
As expected, ablating the task information worsens the performance of both \Gls{maml-concat} and \gls{maml-context}.
Further, ablating phase information (Figure \ref{fig:regression_ablation}, left panel) affects the performance more compared to ablating amplitude information (Figure \ref{fig:regression_ablation}, right panel).
Next, \gls{maml-concat}'s performance worsens more compared to \gls{maml-context} in both experiments suggesting that context-conditioning is more robust to noisy or partial context information.
Importantly, in both experiments, the performance of \gls{maml-context} is still significantly better than \gls{maml} whereas \gls{maml-concat} is not better when phase information is ablated (refer to the plot of \gls{maml} in Figure~\ref{fig:regression} for comparison), suggesting that context conditioning on even partial task information is useful in reducing task ambiguity.

\paragraph{Extrapolation.} We next compare the extrapolation performance of the different methods by sampling an amplitude from $[5.  0, 10.  0]$, \ie outside the range given during meta-training, $[0.  1, 5.  0]$.
The performance of \gls{maml-context} is greater than the performance of \gls{maml} again, showing the benefit of context-conditioning (refer to Figure \ref{fig:regression_extrapolation}).
Interestingly, we see that \gls{maml-concat} performs worse than all other methods and the extra parameter-count baseline \gls{maml-static} is quite competitive and performs similarly to \gls{maml-context}, suggesting that the context network is still sensitive to the distribution of task information observed in training.
In hindsight, this is to be expected, as the meta-learning formulation makes the assumption that meta-training and meta-evaluation tasks are drawn from the same distribution.


==> data/cub.tex <==
shot,maml-mean,maml-std,dynamic-mean,
3,0.5154444575309753,,
5,0.5684221982955933,,0.5536666512489319

==> figures/exp_birds.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.6\textwidth}
  \begin{subfigure}{\textwidth}
    \centering
    \begin{tabular}{p{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}}
      \resizecrop{{figures/cub/American_Three_Toed_Woodpecker_0030_796144}.jpg} &
      \resizecrop{{figures/cub/Prothonotary_Warbler_0105_174097}.jpg} &
      \resizecrop{{figures/cub/Song_Sparrow_0042_121314}.jpg} &
      \resizecrop{{figures/cub/Black_Footed_Albatross_0002_55}.jpg} &
      \resizecrop{{figures/cub/Red_Cockaded_Woodpecker_0025_794710}.jpg}
    \end{tabular}
    \caption{Support set examples; $k$-shot classification provides $k$ of each class.}
  \end{subfigure}

  \begin{subfigure}[b]{.75\textwidth}
    \tiny
    \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{l}
      \texttt{spotted body feathers, spotted breast feather, and thin beak} \\ 
      \texttt{intensely yellow body and bluish grey wings} \\ 
      \texttt{white bird with black stripes on the breast and wingbars} \\ 
      \texttt{brown in color with a long curved beak and dark eye rings} \\ 
      \texttt{wings that are spotted and has a white molar patch} 
    \end{tabular}
    \caption{Task information (a set of descriptions for each class).}
  \end{subfigure}
  \hspace{1pt}
  \begin{subfigure}[b]{.18\textwidth}
    \begin{tabular}{c}
      \resizecrop{{figures/cub/Prothonotary_Warbler_0107_173921}.jpg}
    \end{tabular}
    \caption{A query.}
  \end{subfigure}

\label{fig:cub-data}
\end{subfigure}%
\hspace{1pt}
\begin{subfigure}{.35\textwidth}
  \centering
    \begin{tikzpicture}%
      \begin{axis}[%
        acc-over-shot,
        ymin=40,
        ymax=60,
      ]

      \addplot[
        color=green,
        %mark=square,
      ]
      coordinates {
        (1,0) (2,0) (3,0) (4,0) (5,55.27)
      };
      \label{plot:maml}
      \addlegendentry{\acrshort{maml}}

      \addplot[
        color=black,
        %mark=square,
      ]
      coordinates {
        (1,0) (2,0) (3,0) (4,0) (5,57.68)
      };
      \label{plot:maml-static}
      \addlegendentry{\gls{maml-static}}

      \addplot[
        color=blue,
        %mark=square,
      ]
      coordinates {
        (1,0) (2,0) (3,0) (4,0) (5,0)
      };
      \label{plot:maml-concat}
      \addlegendentry{\gls{maml-concat}}

      \addplot[
        color=red,
        %mark=square,
      ]
      coordinates {
        (1,46.24) (2,52.95) (3,55.42) (4,58.3) (5,59.73)
      };
      \label{plot:maml-dynamic}
      \addlegendentry{\gls{maml-dynamic}}

    \end{axis}

    \end{tikzpicture}%

  \caption{
    Average meta-test-set accuracy 
    as the number of support set examples is increased.
  }
  \label{fig:cub-acc}
\end{subfigure}
\label{fig:cub}
\caption{
  The \glsfirst{cub} few-shot learning task.
}
\end{figure*}


==> figures/exp_regression.tex <==
\begin{figure*}[t]
\begin{subfigure}[b]{.2\linewidth}
\hspace{-4pt}
\begin{tikzpicture}%
  \begin{axis}[%
    avg-loss,
    ylabel={validation loss},
    xmin=0,xmax=5000,
    ymin=0.001,
    ymode=log,
    log ticks with fixed point,
    y tick label style={/pgf/number format/1000 sep=\,},
  ]

  \errorband{data/sinusoid/sinusoid-maml.csv}{iteration}{mean}{std}{black}{0.4}
  %\addlegendentry{\gls{maml} \\ (base)}

  \errorband{data/sinusoid/sinusoid-static.csv}{iteration}{mean}{std}{black!15!green}{0.4}
  %\addlegendentry{\gls{maml-static} \\ (ablation)}

  \errorband{data/sinusoid/sinusoid-concat.csv}{iteration}{mean}{std}{blue}{0.4}
  %\addlegendentry{\gls{maml-concat} \\ (strong baseline)}

  \errorband{data/sinusoid/sinusoid-context.csv}{iteration}{mean}{std}{orange}{0.4}
  %\addlegendentry{\gls{maml-context} \\ \textbf{(ours)}}

  \end{axis}
\end{tikzpicture}%

\vspace{-5pt}
\centering{\scriptsize\phantom{meta-training iterations}}

\caption{
  Fully observable task information.
}
\label{fig:regression}
\end{subfigure}
%
\hspace{12pt}
%
\begin{subfigure}[b]{.37\linewidth}
\hspace{-4pt}
\begin{tikzpicture}
  \begin{axis}[%
    avg-loss,
    xmin=0,xmax=5000,
    ymin=0.001,
    ymode=log,
    log ticks with fixed point,
    y tick label style={/pgf/number format/1000 sep=\,},
  ]

  \errorband{data/sinusoid/sinusoid-ablate-phase-concat.csv}{iteration}{mean}{std}{blue}{0.4}
  %\addlegendentry{\gls{maml-concat} \\ (ablate phase)}

  \errorband{data/sinusoid/sinusoid-ablate-phase-context.csv}{iteration}{mean}{std}{orange}{0.4}
  %\addlegendentry{\gls{maml-context} \\ (ablate phase)}

  \end{axis}
\end{tikzpicture}%
%
\begin{tikzpicture}
  \begin{axis}[%
    avg-loss,
    xmin=0,xmax=5000,
    ymode=log,
    ymin=0.001,
    log ticks with fixed point,
    y tick label style={/pgf/number format/1000 sep=\,},
  ]

  %\addplot+[black,thin,dashed,no markers] table [col sep=comma, x=iteration, y=mean] {data/sinusoid/sinusoid-maml.csv};
  %%\addlegendentry{\gls{maml}}

  %%\errorband{data/sinusoid/sinusoid-static.csv}{iteration}{mean}{std}{black!15!green}{0.4}
  %%\addlegendentry{\gls{maml-static}}

  %\addplot+[blue,thin,dashed,no markers] table [col sep=comma, x=iteration, y=mean] {data/sinusoid/sinusoid-concat.csv};
  %%\addlegendentry{\gls{maml-concat}}

  %\addplot+[orange,thin,dash pattern=on 1pt off 0.5pt on 1pt off 0.5pt,no markers] table [col sep=comma, x=iteration, y=mean] {data/sinusoid/sinusoid-context.csv};
  %%\addlegendentry{\gls{maml-context}}

  \errorband{data/sinusoid/sinusoid-ablate-amplitude-concat.csv}{iteration}{mean}{std}{blue}{0.4}
  %\addlegendentry{\gls{maml-concat} \\ (ablate amplitude)}

  \errorband{data/sinusoid/sinusoid-ablate-amplitude-context.csv}{iteration}{mean}{std}{orange}{0.4}
  %\addlegendentry{\gls{maml-context} \\ (ablate amplitude)}

  \end{axis}
\end{tikzpicture}%

\vspace{-5pt}
\hspace{15pt}
\centering{\scriptsize\textbf{meta-training iterations}}

\caption{
  Partial information with 
  (\textbf{left}) phase or (\textbf{right}) amplitude ablated.
}
\label{fig:regression_ablation}
\end{subfigure}
%
\hspace{8pt}
%
\begin{subfigure}[b]{.3\linewidth}
\begin{tikzpicture}%
  \begin{axis}[%
    avg-loss,
    xmin=0,xmax=5000,
    ymode=log,
    log ticks with fixed point,
    y tick label style={/pgf/number format/1000 sep=\,},
  ]

  \errorband{data/sinusoid/sinusoid-maml-extrapolation.csv}{iteration}{mean}{std}{black}{0.4}
  \addlegendentry{\gls{maml} (base)}

  \errorband{data/sinusoid/sinusoid-static-extrapolation.csv}{iteration}{mean}{std}{black!15!green}{0.4}
  \addlegendentry{\gls{maml-static} \\ (ablation)}

  \errorband{data/sinusoid/sinusoid-concat-extrapolation.csv}{iteration}{mean}{std}{blue}{0.4}
  \addlegendentry{\gls{maml-concat} \\ (strong baseline)}

  \errorband{data/sinusoid/sinusoid-context-extrapolation.csv}{iteration}{mean}{std}{orange}{0.4}
  \addlegendentry{\gls{maml-context} \textbf{(ours)}}

  \end{axis}
\end{tikzpicture}%

\vspace{-5pt}
\centering{\scriptsize\phantom{meta-training iterations}}

\caption{
  Extrapolation (amplitude sampled outside the range) study.
}
\label{fig:regression_extrapolation}
\end{subfigure}

\caption{
  Mean and standard deviation of the per-task validation loss over meta-training iterations, in log scale, 
  on the sinusoidal regression task set described in Section \ref{sec:sinusoid}.
}
\end{figure*}


==> figures/fig_explanatory.tex <==
\begin{figure*}[t]  \includegraphics[width=1\linewidth]{figures/fig_explanatory1}
  \caption{
  \textbf{Overview of our approach.} 
\textbf{(a)} Standard approaches to meta-learning estimate a global parameter $\metaparams$ that is used to constrain the learning of local parameters $\taskparams$ in a task-agnostic manner; \ie, the value of $\metaparams$ for each task-specific $\taskparams$ does not depend on properties of the task in question.
%
\textbf{(b)} Consider a child raised in a bilingual home. In this environment, contextual cues (\eg the face of the mother or father) serve as a prime to guide the child to learn labels for unseen objects (such as dogs and cats) in the appropriate language~\citep[example adapted from][]{werchan20158}. Thus, in contrast to standard meta-learning, learning-to-learn in humans is guided by contextual cues. \textbf{(c)} We investigate whether using task-specific contextual information can be leveraged in meta-learning by learning an initialization of the task-specific model parameters $\taskparams$ as a function of the task information $\context$.}
\label{fig:explain}
\end{figure*}
